Graph Neural Network Policies and Imitation Learning for Multi-Domain Task-Oriented Dialogues

Task-oriented dialogue systems are designed to achieve specific goals while conversing with humans. In practice, they may have to handle simultaneously several domains and tasks. The dialogue manager must therefore be able to take into account domain changes and plan over different domains/tasks in order to deal with multidomain dialogues. However, learning with reinforcement in such context becomes difficult because the state-action dimension is larger while the reward signal remains scarce. Our experimental results suggest that structured policies based on graph neural networks combined with different degrees of imitation learning can effectively handle multi-domain dialogues. The reported experiments underline the benefit of structured policies over standard policies.

==> sections/approach/box_01_annexe.tex <==

Let $n$ be the number of slots and $L$ the number of layers. Let be $\mathbf{x}$ the belief state, $\mathbf{x}_0=\phi_0(x)$, $\mathbf{h}^l_0\, \forall l\in[0,L-1]$ and $\mathbf{y}_0$ be the successive \textsc{I-node} representations. Let the successive \textsc{S-nodes} representations be $\forall i \in[1,n], \, \mathbf{x}_i=\phi_i(x)$, $\mathbf{h}^l_i\ \forall l\in[0,L-1]$ and $\mathbf{y}_i$. First, the \textsc{GNN} transforms inputs:
\begin{equation}
\begin{split}
    \forall i \in [0, n],\quad \mathbf{h}^0_i = F_i^0(\phi_i(\mathbf{x})) \\
    \mathrm{with}\quad F_i^0(\mathbf{h}) = \sigma^0(\mathbf{W}_i^0\mathbf{h} + \mathbf{b}_i^0)
\end{split}
\end{equation}
Then, at the $l$-th layer, it computes the internal nodes representations (Eq.~\ref{eq:internal}) by following message sending\footnote{The notation $i \leftarrow j$ is to denote a message sending from slot $j$ to slot $i$. It also corresponds to the directed relation between the slots $j$ and $i$. The notation $i \leftarrow *$ is to denote all messages sending to slot $i$.} (Eq.~\ref{eq:send}), message aggregation (Eq.~\ref{eq:agg}) and representation update (Eq.~\ref{eq:update}):
\begin{subequations}
\begin{align}
    %\forall l \in [1, L-1],\quad 
    & \forall i \in [0, n],\quad \mathbf{h}^{l}_{i} = F_i^l(\mathbf{h}^{l-1}) \label{eq:internal} \\
    \mathbf{m}^{l}_{i \leftarrow j} & = M_{i \leftarrow j}^l(\mathbf{h}^{l-1}_{j}) % = \mathbf{W}_{i \leftarrow j}^l \mathbf{h}^{l-1}_{j} + \mathbf{b}^{l}_{i \leftarrow j}
    \label{eq:send} \\
    \mathbf{m}^{l}_{i} & = A_i^l(\mathbf{m}^{l}_{i \leftarrow *}) \label{eq:agg} \\
    \mathbf{h}^{l}_{i} & = U_i^{l}(\mathbf{m}^{l}_{i}) =  \sigma^{l}(\mathbf{m}^{l}_{i}  \label{eq:update})
\end{align}
\end{subequations}
The message sending function $M_{i \leftarrow j}^l$ is a linear transformation with bias. 
The message aggregation function $A_i^l$ is the average pooling function.
The representation update function $U_i^{l}$ compute the new hidden representation with \textsc{ReLU} activation function and dropout technique during learning stage.
Finally, the \textsc{GNN} concatenates ($\oplus$ symbol) all final nodes representations and computes the value or policy functions depending on the final activation function (linear or softmax).
\begin{gather}
    \mathbf{y} = \sigma^L(\bigoplus_{i=0}^n \mathbf{W}_{i}^L \mathbf{h}_i^{L-1} + \mathbf{b}_i^{L})
\end{gather}

%\paragraph{\textsc{GNN}: Adjacency matrix view}

%Let $\mathbf{A}_k$ be the adjacency matrix to represent the graph w.r.t the relation $k$ ($i \leftarrow j = k$ if $\mathbf{A}_k[i,j]\neq0$), $\mathbf{H}^l$ the state vectors of nodes in time step $l$ into a matrix. 
%The adjacency matrices are not used explicitly in the forward module here but they have an influence of the choice of weight $\mathbf{W}_{i \leftarrow j}^l$.\footnote{If there are more than one relation between the slots $j$ and $i$, it is possible to consider relation aggregation. But it is not in the scope of our research. By default, it is the sum aggregation.}

% Let $\mathbf{H}^l$ the state vectors of nodes in time step $l$ into a matrix.
% By using the sum aggregation function in any place, it is equivalent to:
%\begin{gather}
%    \mathbf{H}^{l} = \sigma^l(\sum_k \mathbf{W}_{k}^l \mathbf{H}^{l-1} \mathbf{A}_{k})
%\end{gather}

% We consider $A_k$ as the fixed (or given) adjacency matrix for the $k^{th}$ specific relation. As shown previously, we have 5 relations: I, S, S2I, S2S and I2S.

==> sections/approach/box_04.tex <==
\todo{Present prototypes here.}


==> sections/approach/box_05.tex <==
\paragraph{Baseline}

% \todo{Please move it to experiments}

The baseline is a classical feed-forward neural network (or multi-layer perceptron). The belief state with summary representation is considered in such a way that all information is contained in a single input vector. Similarly, the probabilistic distribution over all possible actions is based on a single output vector with its summary representation.

To draw a parallel with DIP representation, it is as if all the slot-dependent and slot-independent representations have been concatenated into a single vector (see Figure \ref{sub:model_fnn} and \ref{sub:model_stnn}).

Let $\mathbf{x}$ be the input and $\mathbf{y}$ the output. Let $\mathbf{x}$, $\mathbf{h}^l \, \forall l\in[0,L-1]$ and $\mathbf{y}$ be the successive representations of belief state.

\paragraph{Input Module}
\begin{subequations}
\begin{gather}
    \mathbf{h}^0 = F^0(\phi(\mathbf{x})) \\ % \approx F^0(\mathrm{onehot}(\mathbf{x}))
    \mathrm{with}\quad F^0(\mathbf{h}) = \sigma^0(\mathbf{W}^0\mathbf{h} + \mathbf{b}^0)
\end{gather}
\end{subequations}

\paragraph{Forward Module}
\begin{subequations}
\begin{gather}
    \forall l \in [1, L-1],\quad \mathbf{h}^{l} = F^{l}(\mathbf{h}^{l-1}) \\
    \mathrm{with}\quad F^{l}(\mathbf{h}^{l-1}) = \sigma^{l}(\mathbf{W}^l \mathbf{h}^{l-1} + \mathbf{b}^l)
\end{gather}
\end{subequations}

\paragraph{Output Module}
\begin{gather}
    \mathbf{y} = \sigma^{L}(\mathbf{W}^L \mathbf{h}^{L-1} + \mathbf{b}^L)
\end{gather}

==> sections/approach/fig_01.tex <==
\begin{figure*}[ht!]
  \begin{center}
    \subfloat[Classical FNN representation.]{
        \includegraphics[width=0.28\textwidth]{figures/approach/model_1.png}
        \label{sub:model_fnn}
    }\hspace{0.04\textwidth}
    \subfloat[FNN representation with DIP.]{
        \includegraphics[width=0.28\textwidth]{figures/approach/model_2.png}
        \label{sub:model_stnn}
    }\hspace{0.04\textwidth}
    \subfloat[GNN representation with DIP.]{ %  (symmetries are produced by slot permutation invariance)
        \includegraphics[width=0.28\textwidth]{figures/approach/model_3.png}
        \label{sub:model_gnn}
    }\\
    %\subfloat[Hierarchical GNN for composite dialogues. On the left, the hierarchical decision loads the specific GNN that makes the final action decision. On the left, the GNN is shared between all domains.]{
    %    \includegraphics[width=0.9\textwidth]{figures/approach/hierarchy.png}
    %    \label{sub:hierarchy}
    %}\\
  \end{center}
  \caption{Structures of the neural network layers. The central box represents the weight matrix of a layer. It can be decomposed into sub-matrices according to the graph structure assumption. The left circles represent the state vectors of the slots as the input of the network (it can be the concatenation of all the vectors of the slots or a collection of sub-vectors). The right circles represent the action vectors of the slots at the output of the network.}
  \label{fig:models}
\end{figure*}

==> sections/conclusion/box_01.tex <==
what can you said about the distinct evaluations, what the results suggest? what are the insights or intuitions behind the results, how can you explain the results?


Our main contribution is to study how structured policies like \textsc{GNN} combined with some imitation learning can be effective to handle multi-domain dialogues.
%and how they can be robust face to sparse rewards due to composite dialogues.
We provide large scale experiments, in which we analyze the performance of different type of policies, from single-domain policies to generic ones, with different \textsc{RL} algorithms and different levels of imitation learning.
These experiments underline the clear benefit of structured policies against naive feed-forward policies.
%when structuring decision-making with a naive hierarchical decomposition.
%Then, we propose to study the learning effectiveness of these approaches with imitation learning in order to emphasize the importance of structuring the dialogue policy.
Finally, we evaluate the best approach in a full dialogue pipeline with simulated and real users to validate these claims in practice.

==> sections/conclusion/box_02.tex <==
The idea is to have the scalability property to have a hierarchical decision policy at the multi-domain level without depending on the number of domains. It could be interesting to have a multi-domain independent parameterization (MDIP) and to use feudal learning at multi-domain level but it is out of the scope of this paper.
%LINA >>> If it is out of the scope of the paper then don't even talk about it, move it to future work.

==> sections/evaluation/box_01.tex <==
The results of the evaluation of single-domain dialogues are presented in Table~\ref{tab:sotatablepydial}.
We observe that our \textsc{ACGNN} proposal achieves competitive performance in the long training stage in environments with action masking mechanism and with semantic error rates\footnote{This corresponds to the noise that comes from the \textsc{NLU} and \textsc{NLG} channels.} of $0\%$, $15\%$ and $30\%$ for respectively \textsc{Env1}, \textsc{Env3} and \textsc{Env6}.
\textsc{ACGNN} is better than \textsc{DQNGNN} in a majority of environments. But it seems that our proposal is less efficient when the action masking mechanism is not activated (in \textsc{Env2} and \textsc{Env4}).
\textsc{ACGNN} certainly remains more limited against \textsc{STRAC} in the short training stage and in unfriendly environment like \textsc{Env5} since the latter has more advanced learning mechanisms. Our approach manages to reach a performance close to or even better than those of \textsc{STRAC} and those of \textit{handcrafted} (\textsc{HDC}) policies.
This confirms that our structured policies are suitable for single-domain task-oriented dialogues.


==> sections/evaluation/box_02.tex <==
Concerning the re-evaluation of the proposed policies in \textsc{ConvLab}, the results of success rates are presented in Figure~\ref{subfig:convlab_bench}.
All baselines have difficulties to learn on a horizon of $10\,000$ dialogues with a clear stagnation of the success rate between $0\%$ and $20\%$. 
This is evidence of the difficulties of learning with sparse rewards on multi-domain dialogues.


==> sections/evaluation/box_04.tex <==
From now on, we decide to use \textsc{ACER} with shared-\textsc{GNN} and \textsc{ILfOS} under the name \textsc{\textbf{ACGOS}}. %\textbf{ACGNN}.
We train it with a horizon of $100\,000$ dialogues and compare it with baselines proposed by \citet{rohmatillah2021corrective} that they are pre-trained with \textsc{BC} without mentioning the total number of training dialogues. The results of this long training stage are presented in Table~\ref{tab:policytableconvlab} and confirm that out method is competitive with baselines.


==> sections/experiments/figure_convlab_bench.tex <==
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=0.5\textwidth]{figures/results/success_BENCH.png}
    \caption{Distribution of the performance of the baselines on multi-domain dialogues in \textsc{ConvLab}, with 10 random initializations. The colored area represents the distribution and the middle line represents its median.}
    \label{fig:convlab_bench}
  \end{center}
\end{figure}

==> sections/experiments/old/figure_convlab_a2c.tex <==
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/results/success_A2C.png}
    \caption{TODO}
    \label{fig:convlab_a2c}
  \end{center}
\end{figure}

==> sections/experiments/old/figure_convlab_a2cilfod.tex <==
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/results/success_A2CILFOD.png}
    \caption{TODO}
    \label{fig:convlab_a2cilfod}
  \end{center}
\end{figure}

==> sections/experiments/old/figure_convlab_a2cilfos.tex <==
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/results/success_A2CILFOS.png}
    \caption{TODO}
    \label{fig:convlab_a2cilfos}
  \end{center}
\end{figure}

==> sections/experiments/old/figure_convlab_bc.tex <==
\begin{figure}[ht!]
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/results/success_BC.png}
    \caption{TODO}
    \label{fig:convlab_bc}
  \end{center}
\end{figure}

==> sections/experiments/table_convlab_full.tex <==
\begin{table*}[!htb]
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{ccc|ccccccccc}
    \toprule
    \multicolumn{3}{c|}{\textbf{Configuration}} & \textbf{Avg Turn} & \textbf{Inform (\%)} & \textbf{Book} & \multicolumn{2}{c}{\textbf{Complete}} & \multicolumn{2}{c}{\textbf{Success}} \\
    \textbf{NLU} & \textbf{Policy} & \textbf{NLG} &  \textbf{(succ/all)} & \textbf{Prec. / Rec. / F1} & \textbf{Rate (\%)} & \multicolumn{2}{c}{\textbf{Rate (\%)}} & \multicolumn{2}{c}{\textbf{Rate (\%)}} \\
    \midrule \midrule
    -  & HDC & - & 10.6/10.6 & 87.2 / 98.6 / 90.9 & 98.6 & 97.9 & - & 97.3 & - \\
    -     & ACGOS (ours) & -        & 13.1/13.2 & 94.8 / 99.0 / 96.1 & 98.7 & 98.2 & (+0.3) & 97.0 & (-0.3) \\ 
    \midrule
    \textsc{BERT}  & HDC & T & 11.4/12.0 & 82.8 / 94.1 / 86.2 & 91.5 & 92.7 & - & 83.8 & - \\
    \textsc{BERT}  & HDC$^{\dagger}$ & T & 11.6/12.3 & 79.7 / 92.6 / 83.5 & 91.1 & 90.5 & (-2.2) & 81.3 & (-2.5) \\
    %\textsc{BERT}  & \textsc{ACGOS} (ours) & T & 14.0/14.8 & 76.2 / 92.2 / 80.8 & 87.0 & 88.5 & 74.8 \\
    \textsc{BERT}  & \textsc{MLE}*  & T & 12.2/----- & ----- / ----- / 67.8 & ----- & 46.7 & (-46.0) & 41.9 & (-41.9) \\
    \textsc{BERT}  & \textsc{MLE}$^{\dagger}$  & T & 12.1/24.1 & 62.8 / 69.8 / 62.9 & 17.6 & 42.7 & (-50.0) & 35.9 & (-47.9) \\
    \textsc{BERT}  & \textsc{PG}*   & T & 12.5/----- & ----- / ----- / 67.1 & ----- & 47.6 & (-45.1) & 42.0 & (-41.8) \\
    \textsc{BERT}  & \textsc{PG}$^{\dagger}$   & T & 11.0/25.3 & 57.4 / 63.7 / 56.9 & 17.4 & 37.4 & (-55.3) & 31.7 & (-52.1) \\
    \textsc{BERT}  & \textsc{GDPL}* & T & 12.2/----- & ----- / ----- / 67.9 & ----- & 49.9 & (-42.8) & 44.0 & (-39.8) \\
    \textsc{BERT}  & \textsc{GDPL}$^{\dagger}$ & T & 11.5/21.3 & 64.5 / 73.8 / 65.6 & 20.1 & 49.4 & (-43.3) & 38.4 & (-45.4) \\
    \textsc{BERT}  & \textsc{PPO}*  & T & 11.6/----- & ----- / ----- / 71.1 & ----- & 64.9 & (-27.8) & 63.8 & (-20.0) \\
    \textsc{BERT}  & \textsc{PPO}$^{\dagger}$  & T & 13.1/17.8 & 69.4 / 85.8 / 74.1 & 86.6 & 75.5 & (-17.2) & 71.7 & (-12.1) \\
    \textsc{BERT}  & \textsc{ACGOS} (ours) & T & 14.0/14.8 & 88.8 / 92.6 / 89.5 & 86.6 & 89.1 & (-3.6) & 81.7 & (-2.1) \\
    \bottomrule
\end{tabular}
}
\caption{Dialogue system evaluation with simulated users and different configurations. T means template-based. Configurations without \textsc{NLU} and \textsc{NLG} modules pass directly the dialogue act. Configurations with \textsc{ACGOS} and HDC policies are been evaluated on a single run with $1\,000$ dialogues.
Maximum likelihood estimation (\textsc{MLE}) is a standard supervised learning method based on the \textsc{MultiWOZ} dataset~\cite{budzianowski2018multiwoz}.
Policy gradient (\textsc{{PG}}) is a standard policy based method.
Proximal policy optimization (\textsc{{PPO}}) \citep{schulman2017proximal} is a more sophisticated actor-critic based method.
Guided dialogue policy learning (\textsc{{GDPL}}) is a join policy optimization and reward estimation method using adversarial inverse reinforcement learning \citep{takanobu2019guided}.
Configurations with * are taken from \citet{rohmatillah2021corrective} and used behaviour cloning as the pre-trained weights. Configurations with ${\dagger}$ are taken from the \href{https://github.com/thu-coai/ConvLab-2/tree/ad32b76022fa29cbc2f24cbefbb855b60492985e}{GitHub of \textsc{ConvLab}}. \textsc{PPO} in \textsc{ConvLab} used behaviour cloning as the pre-trained weights (see the \href{https://github.com/thu-coai/ConvLab-2/issues/54 }{issue "RL policy training" in GitHub}).
Some missing information has been noted as  ---.}
\label{tab:sotatableconvlab_2}
\end{table*}


==> sections/experiments/table_convlab_human.tex <==
\begin{table}[!tb]
\centering
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{c|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Configuration}} & \textbf{Avg} 
    & \textbf{Success} & \textbf{Nb of} \\
    & \textbf{Turn} 
    & \textbf{Rate (\%)} & \textbf{Dial.} \\
    \midrule \midrule
    \textsc{BERT} + HDC~\cite{li2020results} & 15.48 
    & 65.81 $\pm$  9.48 & 100 \\
    \textsc{MILU} + HDC~\cite{li2020results} & 17.54 
    & 56.45 $\pm$  9.92 & 100 \\
    \hline
    \textsc{BERT} + \textsc{ACGOS} (Ours) & 17.12  
    & 57.78 $\pm$ 14.73 &  45 \\
    \textsc{MILU} + \textsc{ACGOS} (Ours) & 21.36    
    & 50.06 $\pm$ 14.58 &  47 \\
    \bottomrule
\end{tabular}
}
\caption{Dialogue system evaluation with real users and different configurations and a 95\% confidence level for success rates. Configurations with HDC (for handcrafted policy) are taken from \citet{li2020results}.}
\label{tab:humantableconvlab}
\end{table}


==> sections/experiments/table_convlab_policy.tex <==
\begin{table}[!htb]
\centering
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{cc}
    \toprule
    \textbf{Models} & \textbf{Success Rate (\%)} \\
    \midrule \midrule
    MLE* & 43 \\
    PG* & 48 \\
    GDPL* & 48 \\
    PPO* & 80 \\
    Rule Policy & 96 \\
    \midrule
    \textbf{ACGNN} & \textbf{87.6} \\
    \bottomrule
\end{tabular}
}
\caption{Policy evaluation with different methods from \citet{rohmatillah2021corrective}. * is used when the methods uses BC pre-training. ACGNN was trained with $100\,000$ dialogues and evaluated on $1\,000$ dialogues.}
\label{tab:policytableconvlab}
\end{table}


==> sections/related_work/box_01.tex <==
%\textbf{Dialogue Systems} Single vs. Multi Domain / (non)-Composite 
%LINA: I will temporarily comment this, I don't think we need
%to talk about this in here.

%Dialogue Task / (non)-Distributed Dialogue Task
% ; RL / IL / HL

%; DSTC8 \citep{li2020results} ; DSTC9 \citep{li2021multi} ; Empirical analysis of system-wise evaluation \citep{takanobu2020your}

==> sections/related_work/box_02.tex <==
\label{sec:hrl}
%Fundamental hierarchical reinforcement learning frameworks~\cite{dayan1993feudal,parr1998reinforcement,sutton1999between,dietterich2000hierarchical} have inspired a wide variety of work on dialogue management. Typically, at a high level of abstraction, a meta-controller (or master policy) manages a set of controllers which operate at a lower level (we refer them as \textit{meta-actions} or \textit{sub-policies}). We focus on space abstraction i.e how to decompose the decision-making process from state space to action space.

Hierarchical reinforcement learning is used by dialogue manager
to delegates the low-level dialogue actions to sub-policies.
%to share slot management between sub-policies.
For instance, the \textit{feudal} hierarchy has been combined with actor actor-critic with experience replay (ACER) and with deep Q-learning network (DQN) in ~\citet{casanueva2018feudal, casanueva2018feudal2} by dividing the task into
sub-tasks and the master policy's action chooses a slot-dedicated sub-policy. 
These sub-policies are based on the DIP representation of their corresponding slot and can share weights \citep{wang2015learning, papangelis2019single}.

%So far the space abstraction implies to build independent sub-policies.
So far hierarchical learning implies to build independent sub-policies.
A more structured hierarchy with \textsc{GNN} rather than a set of classical \textit{feed forward networks} (\textsc{FNN}) allows one to build non-independent sub-policies resulting in a more expressive global policy. Another major advantage of structured policies is their modularity (or scalability) and thus their ability to generalize between similar dialogue tasks \citep{chen2018structured, chen2020distributed}.

These hierarchical and structured mechanisms have been used in recent methods: % \textsc{FeudalGain} \citep{geishauser2021does} is based on \textsc{Feudal-ACER} with an intrinsic reward based on information gain and %to favour actions that resolve uncertainty or query the user whenever necessary ; 
for example, \textsc{STRAC} \citep{chen2020distributed} is an \textsc{ACER} variant of \textsc{DQN-GNN} that proposes an implicit policy decomposition and uses noisy networks for exploration.
The purpose of this method was to improve domain adaptation and learning efficiency.
With \textsc{ComNet}, \citet{chen2020structured} were the first to propose a multi-domain dialogue variant of \textsc{DQN-GNN} by adding a domain-selection hierarchy level. For experimental purposes, they  discarded the domain provided by the \textit{dialogue state tracker} (\textsc{DST}) module.
They relied on the \textsc{DIP} to share the same \textsc{GNN} structure for all domain-specific sub-policies and they evaluated their policies in \textsc{PyDial}.



==> sections/related_work/box_03.tex <==
%LINA: temporarily commenting this
%DQfD \citep{hester2018deep}

%IL on dialogues \citep{cordier2020diluted}

%Weak experts learning \citep{gordon2020learning}

%Behavior Cloning with Auxiliary Tasks (for pre-training RL methods in order to alleviate causal confusion problem in BC) + Corrective guidance (for policy improvement) \citep{rohmatillah2021corrective}
